On-Shell Flow

In this work, the problem of constructing geometric flow equations that preserve Einstein field equations for the spacetime metric is addressed. After having briefly discussed the main features of Ricci flow, the on-shell flow equations for a system comprised of a dynamical metric and a set of matter fields are constructed. Then, two examples in which the matter content is just a single, self-interacting scalar field are analysed in detail, imposing the geometric flow equations to be the action-induced ones. In conclusion, an explicit connection to the Swampland Distance Conjecture is proposed.

==> Extra.tex <==
\be
\nabla_\mu\nabla_\nu\phi=\de_\mu\de_\nu\phi-\Gamma^\alpha_{\mu\nu}\de_\alpha\phi
\ee



\be
\begin{split}
    \nabla_\sigma\nabla_\mu\nabla_\nu\phi &=\de_\sigma\de_\mu\de_\nu\phi-\Gamma^\alpha_{\mu\nu}\de_\sigma\de_\alpha\phi-\de_\sigma\Gamma^\alpha_{\mu\nu}\de_\alpha\phi-\Gamma^\alpha_{\sigma\mu}\de_\alpha\de_\nu\phi\\
    &\quad +\Gamma^\alpha_{\sigma\mu}\Gamma^\beta_{\alpha\nu}\de_\beta\phi-\Gamma^\alpha_{\sigma\nu}\de_\mu\de_\alpha\phi+\Gamma^\alpha_{\sigma\nu}\Gamma^\alpha_{\mu\alpha}\de_\alpha\phi
\end{split}
\ee

\be
\begin{split}
    \nabla_\sigma\nabla_\mu\nabla_\nu\phi &=\de_\sigma\de_\mu\de_\nu\phi-\Gamma^x_{\mu\nu}\de_\sigma\phi'-\de_\sigma\Gamma^x_{\mu\nu}\phi'-\Gamma^x_{\sigma\mu}\de_\nu\phi'\\
    &\quad +\Gamma^\alpha_{\sigma\mu}\Gamma^x_{\alpha\nu}\phi'-\Gamma^x_{\sigma\nu}\de_\mu\phi'+\Gamma^\alpha_{\sigma\nu}\Gamma^x_{\mu\alpha}\phi'
\end{split}
\ee

==> extra3.tex <==


The explicit expression for the non-zero components of $S_{\mu\nu}$ can be given as:
\be
\begin{split}
    S_{tt}&=\kappa_0\frac{\kappa_0\left(x^2+2\lambda\right)-2}{4\left(1-\kappa_0\lambda\right)^2}\ ,\\
    S_{xx}&=\frac{\kappa_0}{2-\kappa_0\left(x^2+2\lambda\right)}\ .
\end{split}
\ee
Assuming to work with $\kappa_0=-1$, those simplify as:
\be
\begin{split}
    S_{tt}&=\frac{x^2+2\left(1+\lambda\right)}{4\left(1+\lambda\right)^2}\ ,\\
    S_{xx}&=-\frac{1}{x^2+2\left(1+\lambda\right)}\ .
\end{split}
\ee
Rescaling the flow parameter as $\xi\equiv2\left(1+\lambda\right)$, the above expressions become:
\be
\begin{split}
    S_{tt}&=\frac{x^2+\xi}{\xi^2}\ ,\\
    S_{xx}&=-\frac{1}{x^2+\xi}\ .
\end{split}
\ee
Therefore, the flow equations for the components of the emerging part of energy-momentum tensor $\hat{T}_{\mu\nu}$ with non-trivial flow, setting the initial condition to be $\hat{T}_{\mu\nu}=0$, are:
\be
\begin{split}
    \frac{\de \hat{T}_{tt}}{\de\xi}&=\frac{x^2+\xi}{\xi^2}\ ,\\
    \frac{\de \hat{T}_{xx}}{\de\xi}&=-\frac{1}{x^2+\xi}\ .
\end{split}
\ee
Such equations can be solved as:
\be 
\begin{split}
   \hat{T}_{tt}&=\int_{2}^{\xi}\frac{\diff y}{y}+x\int_{2/x}^{\xi/x}\frac{\diff y}{y^2}=\log{\frac{\xi}{2}}+\frac{\xi-2}{2\xi}x^2 \ ,\\
   \hat{T}_{xx}&=-\int_{2+x^2}^{\xi+x^2}\frac{\diff y}{y}=\log{\frac{x^2+2}{x^2+\xi}}\ .
\end{split}
\ee 
By substituting back the expression for $\xi$ in terms of $\lambda$, we have:
\be 
\begin{split}
   \hat{T}_{tt}&=\log{\left(\lambda+1\right)}+\frac{\lambda x^2}{2\left(\lambda+1\right)} \ ,\\
   \hat{T}_{xx}&=\log{\frac{x^2+2}{x^2+2\left(\lambda+1\right)}}\ .
\end{split}
\ee 
Therefore, we have derived the explicit flow behaviour of the emerging energy-momentum tensor components in $D=2$, with initial Anti-de Sitter and constant scalar with $m=0$, so that the metric and the scalar follow some gradient flow equations while the equations of motion for the metric are kept on shell. Clearly, general relativity is trivial in $D=2$ and poses a simple constraint, but the example still gives us a hint on how the machinery might work in higher dimensions. Figures \ref{fig1} and \ref{fig2} show the flow behaviour explicitly, at different values of the space coordinate $x$.
\begin{figure}[H]\label{fig1}
    \centering
    \includegraphics[width=0.7\linewidth]{Ttt.png}
    \caption{Plot of $\hat{T}_{tt}$ for different values of $x$. As can observed from the figure, the value of the energy-momentum component gets magnified far from the origin. }
\end{figure}
\begin{figure}[H]\label{fig2}
    \centering
    \includegraphics[width=0.7\linewidth]{Txx.png}
    \caption{Plot of $\hat{T}_{xx}$ for different values of $x$. As can observed from the figure, the value of the energy-momentum component gets suppressed far from the origin. }
\end{figure}\newpage
Concerning the trace of the emerging energy-momentum tensor, we obtain:
\be 
\begin{split}
    \hat{T}&=g^{\mu\nu}\hat{T}_{\mu\nu}=\frac{\hat{T}_{xx}}{g_2}-\frac{\hat{T}_{tt}}{g_1}\\
    &=\frac{-2\left(\lambda+1\right)}{x^2+2\left(\lambda+1\right)}\left[\log{\left(\lambda+1\right)}+\frac{\lambda x^2}{2\left(\lambda+1\right)} \right]\\
    &\quad+\left[1+\frac{x^2}{2\left(\lambda+1\right)}\right]\log{\frac{x^2+2}{x^2+2\left(\lambda+1\right)}}\ .
\end{split}
\ee
\begin{figure}[H]\label{fig2}
    \centering
    \includegraphics[width=0.7\linewidth]{T.png}
    \caption{Plot of $\hat{T}$ for different values of $x$. As can observed from the figure, the value of the energy-momentum trace gets pushed to negative values far from the origin. }
\end{figure}




==> scalars.tex <==
%show that GR alone is NOT enough! Except for cosmological constant and Einstein manifolds
In the following section, we move from treating the energy-momentum tensor as a generic symmetric tensorial source for Einstein field equations and try to characterise it in terms of a specific set of fields. Practically, we choose to work with a theory of the form presented in section \ref{theory} and assume its matter content to be comprised of $N$ real scalar fields $\varphi_i$. Therefore, we have that the associated canonically normalised Lagrangian density is:
\begin{equation}
    \mathcal{L}_M=-\sum_{i=1}^N\frac{1}{2}\nabla^\mu\varphi_i\nabla_\mu\varphi_i-\sum_{i,j=1}^N\gamma_{ij}\varphi_i\varphi_j\ .
\end{equation}
The precise form of the energy-momentum tensor can be shown to be:
\begin{equation}
    \begin{split}
        T_{\mu\nu}&=\sum_{i=1}^N\nabla_\mu\varphi_i\nabla_\nu\varphi_i-g_{\mu\nu}\left(\sum_{i=1}^N\frac{1}{2}\nabla^\alpha\varphi_i\nabla_\alpha\varphi_i+\sum_{i,j=1}^N\gamma_{ij}\varphi_i\varphi_j\right)\ .
    \end{split}
\end{equation}
At this point, considering the flow equations presented in \eqref{floweq}, we assume to work with the metric flow source:
\be 
\begin{split}\label{mss}
     A_{\mu\nu}&\equiv -2R_{\mu\nu}+2\vartheta Rg_{\mu\nu}+\sum_{j=1}^N b_j\nabla_\mu\nabla_\nu\varphi_j+g_{\mu\nu}\sum_{j=1}^N d_j\Delta\varphi_j\ .
\end{split}
\ee 
Its trace is simply:
\begin{equation}
    A=2\left(D\vartheta-1\right)R+\sum_{j=1}^N\left(Dd_j+b_j\right)\Delta\varphi_j\ .
\end{equation}
At this point, by leaving the flow source $C$ for the cosmological constant implicit, we can derive the explicit for $B_{\mu\nu}$ by plugging everything into the expression \eqref{onshellB}
\be\label{osbs}
\begin{split}
   2B_{\mu\nu}&=-2\nabla^\sigma\nabla_\nu R_{\mu\sigma}+2\left[1+\left(2-D\right)\vartheta\right]\nabla_\mu\nabla_\nu R+2\Delta R_{\mu\nu}\\
&\quad-2\nabla_\mu\nabla^\sigma R_{\sigma\nu}+\left[2\left(D-2\right)\vartheta-1 \right]g_{\mu\nu}\Delta R\\
    &\quad+2R_\mu{}^\sigma{}_\nu {}^\theta R_{\sigma\theta}+2RR_{\mu\nu}-2R_\mu{}^\sigma R_{\sigma\nu}-4\Lambda R_{\mu\nu}\\
    &\quad+2\left(C-R_{\sigma\theta}R^{\sigma\theta}+2\Lambda\vartheta R\right)g_{\mu\nu}+\sum_{j=1}^N\Omega^{\ j}_{\mu\nu}\varphi_j\ ,
\end{split}
\ee
where we have defined $N$ metric-dependent differential operators:
\be 
\begin{split}
    \Omega^{\ j}_{\mu\nu}&= b_j\nabla_\mu\nabla^2\nabla_\nu-\left[\left(D-2\right)d_j+b_j\right]\nabla_\mu\nabla_\nu\Delta- b_j\Delta\nabla_\mu\nabla_\nu\\
    &\quad+ \left[b_j\left(2\Lambda\delta_\mu{}^\sigma\delta_\nu{}^{\theta}+g_{\mu\nu}R^{\sigma\theta}\right)\nabla_\sigma\nabla_\theta\right]+ b_j\nabla^\sigma\nabla_\nu \nabla_\mu\nabla_\sigma\\
    &\quad+g_{\mu\nu}\left\{\left[\left(D-2\right)d_j+b_j\right]\Delta\Delta-b_j\nabla^\sigma\nabla^\theta\nabla_\sigma\nabla_\theta+2d_j\Lambda\Delta\right\}\\
    &\quad+\left[\left(R_\mu{}^\sigma\delta_\nu{}^{\theta}-R_\mu{}^\sigma{}_\nu {}^\theta-R\delta_\mu{}^\sigma\delta_\nu{}^{\theta}\right) b_j\nabla_\sigma\nabla_\theta\right]\ .
\end{split}
\ee
The details of the above computation can be found in appendix \ref{compute}.
\subsection{Single scalar field}
By assuming to work with a single scalar field $\phi$, the metric flow source reduces to:
\be\label{singsource}
     A_{\mu\nu}\equiv -2R_{\mu\nu}+2\vartheta Rg_{\mu\nu}+ b\nabla_\mu\nabla_\nu\phi+g_{\mu\nu}d\Delta\phi\ .
\ee
Consequently, the energy-momentum tensor flow source gets to be
\be\label{osbssi}
\begin{split}
   2B_{\mu\nu}&=-2\nabla^\sigma\nabla_\nu R_{\mu\sigma}+2\left[1+\left(2-D\right)\vartheta\right]\nabla_\mu\nabla_\nu R+2\Delta R_{\mu\nu}\\
&\quad-2\nabla_\mu\nabla^\sigma R_{\sigma\nu}+\left[2\left(D-2\right)\vartheta-1 \right]g_{\mu\nu}\Delta R\\
    &\quad+2R_\mu{}^\sigma{}_\nu {}^\theta R_{\sigma\theta}+2RR_{\mu\nu}-2R_\mu{}^\sigma R_{\sigma\nu}-4\Lambda R_{\mu\nu}\\
    &\quad+2\left(C-R_{\sigma\theta}R^{\sigma\theta}+2\Lambda\vartheta R\right)g_{\mu\nu}+\Omega_{\mu\nu}\phi\ ,
\end{split}
\ee
with the differential operator:
\be 
\begin{split}
    \Omega_{\mu\nu}&= b\nabla_\mu\nabla^2\nabla_\nu-\left[\left(D-2\right)d+b\right]\nabla_\mu\nabla_\nu\Delta- b\Delta\nabla_\mu\nabla_\nu\\
    &\quad+ \left[b\left(2\Lambda\delta_\mu{}^\sigma\delta_\nu{}^{\theta}+g_{\mu\nu}R^{\sigma\theta}\right)\nabla_\sigma\nabla_\theta\right]+ b\nabla^\sigma\nabla_\nu \nabla_\mu\nabla_\sigma\\
    &\quad+g_{\mu\nu}\left\{\left[\left(D-2\right)d+b\right]\Delta\Delta-b\nabla^\sigma\nabla^\theta\nabla_\sigma\nabla_\theta+2d\Lambda\Delta\right\}\\
    &\quad+\left[\left(R_\mu{}^\sigma\delta_\nu{}^{\theta}-R_\mu{}^\sigma{}_\nu {}^\theta-R\delta_\mu{}^\sigma\delta_\nu{}^{\theta}\right) b\nabla_\sigma\nabla_\theta\right]\ .
\end{split}
\ee
Given the analysis performed in \cite{DeBiasio:2022omq}, it can be shown that the flow equation associated to \eqref{singsource} can be derived as the gradient flow of the entropy $\mathcal{F}$-functional:

==> scalars2.tex <==
%show that GR alone is NOT enough! Except for cosmological constant and Einstein manifolds
In the following section, we move from treating the energy-momentum tensor as a generic symmetric tensorial source for Einstein field equations and try to characterise it in terms of a specific set of fields. Practically, we choose to work with a theory of the form presented in section \ref{theory} and assume its matter content to be comprised of $N$ real scalar fields $\varphi_i$. Therefore, we have that the associated canonically normalised Lagrangian density is:
\begin{equation}
    \mathcal{L}_M=-\sum_{i=1}^N\frac{1}{2}\nabla^\mu\varphi_i\nabla_\mu\varphi_i+\sum_{i,j=1}^N\gamma_{ij}\varphi_i\varphi_j\ .
\end{equation}
The precise form of the energy-momentum tensor can be shown to be:
\begin{equation}
    \begin{split}
        T_{\mu\nu}&=\sum_{i=1}^N\nabla_\mu\varphi_i\nabla_\nu\varphi_i-g_{\mu\nu}\left(\sum_{i=1}^N\frac{1}{2}\nabla^\alpha\varphi_i\nabla_\alpha\varphi_i-\sum_{i,j=1}^N\gamma_{ij}\varphi_i\varphi_j\right)\ .
    \end{split}
\end{equation}
At this point, considering the flow equations presented in \eqref{floweq}, we assume to work with the metric flow source:
\be 
\begin{split}\label{mss}
     A_{\mu\nu}&\equiv -2R_{\mu\nu}+2\vartheta Rg_{\mu\nu}+\sum_{j=1}^N b_j\nabla_\mu\nabla_\nu\varphi_j+g_{\mu\nu}\sum_{j=1}^N d_j\Delta\varphi_j\\
     &\quad+\sum_{i,j=1}^N e_{ij}\nabla_\mu\varphi_i\nabla_\nu\varphi_j+g_{\mu\nu}\sum_{i,j=1}^N f_{ij}\nabla_\alpha\varphi_i\nabla^\alpha\varphi_j\ .
\end{split}
\ee 
Its trace is simply:
\begin{equation}
    A=2\left(D\vartheta-1\right)R+\sum_{j=1}^N\left(Dd_j+b_j\right)\Delta\varphi_j+\sum_{i,j=1}^N\left(Df_{ij}+e_{ij}\right)\nabla_\alpha\varphi_i\nabla^\alpha\varphi_j\ .
\end{equation}
At this point, by leaving the flow source $C$ for the cosmological constant implicit, we can derive the explicit for $B_{\mu\nu}$ by plugging everything into the expression \eqref{onshellB}
\be 
\begin{split}\label{souceonesc}
    2B_{\mu\nu}&=-2\nabla^\sigma\nabla_\nu R_{\mu\sigma}+2\left[1+\left(2-D\right)\vartheta\right]\nabla_\mu\nabla_\nu R+2\Delta R_{\mu\nu}\\
&\quad-2\nabla_\mu\nabla^\sigma R_{\sigma\nu}+\left[2\left(D-2\right)\vartheta-1 \right]g_{\mu\nu}\Delta R\\
    &\quad+2R_\mu{}^\sigma{}_\nu {}^\theta R_{\sigma\theta}+2RR_{\mu\nu}-2R_\mu{}^\sigma R_{\sigma\nu}-4\Lambda R_{\mu\nu}\\
    &\quad+2\left(C-R_{\sigma\theta}R^{\sigma\theta}+2\Lambda\vartheta R\right)g_{\mu\nu}+\sum_{j=1}^N\Omega^{\ j}_{\mu\nu}\varphi_j\\
        &\quad     +\sum_{i,j=1}^N\Theta_{\mu\nu}^{\ ij}\nabla_\alpha\varphi_i\nabla^\alpha\varphi_j+\sum_{i,j=1}^N\Sigma_{\mu\nu}^{\sigma\theta ij}\nabla_\sigma\varphi_i\nabla_\theta\varphi_j\ .
\end{split}
\ee
Where we have introduced $N$ metric-dependent differential operators
\be 
\begin{split}
    \Omega^{\ j}_{\mu\nu}&= b_j\nabla_\mu\Delta\nabla_\nu-\left[\left(D-2\right)d_j+b_j\right]\nabla_\mu\nabla_\nu\Delta- b_j\Delta\nabla_\mu\nabla_\nu\\
    &\quad+ \left[b_j\left(2\Lambda\delta_\mu{}^\sigma\delta_\nu{}^{\theta}+g_{\mu\nu}R^{\sigma\theta}\right)\nabla_\sigma\nabla_\theta\right]+ b_j\nabla^\sigma\nabla_\nu \nabla_\mu\nabla_\sigma\\
    &\quad+g_{\mu\nu}\left\{\left[\left(D-2\right)d_j+b_j\right]\Delta\Delta-b_j\nabla^\sigma\nabla^\theta\nabla_\sigma\nabla_\theta+2d_j\Lambda\Delta\right\}\\
    &\quad+\left[\left(R_\mu{}^\sigma\delta_\nu{}^{\theta}-R_\mu{}^\sigma{}_\nu {}^\theta-R\delta_\mu{}^\sigma\delta_\nu{}^{\theta}\right) b_j\nabla_\sigma\nabla_\theta\right]
\end{split}
\ee
and $2N^2$ metric-dependent differential operators:
\be
\Theta_{\mu\nu}^{\ ij}\equiv\left(g_{\mu\nu}\Delta-\nabla_\mu\nabla_\nu \right)\left(Df_{ij}+e_{ij}\right)+2\left(\nabla_\mu\nabla_\nu-g_{\mu\nu}\Delta+\Lambda g_{\mu\nu}\right)f_{ij}\ ,
\ee
\be
\begin{split}
   \Sigma_{\mu\nu}^{\sigma\theta ij}&\equiv \Big[\left(R_\mu{}^\sigma+\nabla_\mu\nabla^\sigma \right)\delta_\nu^{\ \theta}+g_{\mu\nu}R^{\sigma\theta}-g_{\mu\nu}\nabla^\sigma\nabla^\theta -R_\mu{}^\sigma{}_\nu {}^\theta\\
&\quad+\left(2\Lambda-R-\Delta \right)\delta_{\mu}^{\ \sigma}\delta_{\nu}^{\ \theta}+\delta_{\mu}^{\ \sigma}\nabla^\theta\nabla_\nu\Big]e_{ij} \ .
\end{split}
\ee
The details of the above computation can be found in appendix \ref{compute}.
\subsection{Single free scalar field}\label{singlesc}
By assuming to work with a single scalar field $\phi$, the metric flow source reduces to:
\be\label{singsource}
\begin{split}
         A_{\mu\nu}&\equiv -2R_{\mu\nu}+2\vartheta Rg_{\mu\nu}+ b\nabla_\mu\nabla_\nu\phi+g_{\mu\nu}d\Delta\phi\\
     &\quad+e\nabla_\mu\phi\nabla_\nu\phi+fg_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi\ .
\end{split}
\ee
Consequently, the energy-momentum tensor flow source gets to be
\be\label{osbssi}
\begin{split}
   2B_{\mu\nu}&=-2\nabla^\sigma\nabla_\nu R_{\mu\sigma}+2\left[1+\left(2-D\right)\vartheta\right]\nabla_\mu\nabla_\nu R+2\Delta R_{\mu\nu}\\
&\quad-2\nabla_\mu\nabla^\sigma R_{\sigma\nu}+\left[2\left(D-2\right)\vartheta-1 \right]g_{\mu\nu}\Delta R\\
    &\quad+2R_\mu{}^\sigma{}_\nu {}^\theta R_{\sigma\theta}+2RR_{\mu\nu}-2R_\mu{}^\sigma R_{\sigma\nu}-4\Lambda R_{\mu\nu}\\
    &\quad+2\left(C-R_{\sigma\theta}R^{\sigma\theta}+2\Lambda\vartheta R\right)g_{\mu\nu}+\Omega_{\mu\nu}\phi\\
    &\quad     +\Theta_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi+\Sigma_{\mu\nu}^{\sigma\theta}\nabla_\sigma\phi\nabla_\theta\phi\ .
\end{split}
\ee
Given the analysis performed in \cite{DeBiasio:2022omq}, we now want to find an entropy $\mathcal{F}$-functional
\begin{equation}\label{funk}
        \mathcal{F}_{\left(\alpha,\gamma\right)}\left(g,\phi\right)=\int\diff^{D}x\sqrt{g}e^{-\phi}\left[R+\alpha\left(\nabla\phi\right)^2+\gamma\Delta\phi\right]
\end{equation}
such that the flow sourced by \eqref{singsource} can be derived as its associated gradient flow equation for $g_{\mu\nu}$ and $\phi$. As discussed in the above-mentioned reference, we have that the volume-preserving gradient of \eqref{funk} gives:
\begin{equation}\label{geneqm}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}+2\left(1-\alpha+\gamma\right)\nabla_{\mu}\phi\nabla_{\nu}\phi-2\left(1+2\gamma\right)\nabla_{\nu}\nabla_{\mu}\phi+\\
        &+2\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\Delta\phi-2\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\left(\nabla\phi\right)^2\ ,
            \end{split}
\end{equation}
\begin{equation}\label{geneqs}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-R+\left[\left(1-\alpha\right)\left(1-D\right)+\gamma\left(1+\frac{D}{2}\right)\right]\left(\nabla\phi\right)^{2}+\\
        &-\left[1-D\left(1-\alpha\right)+\gamma\left(2+\frac{D}{2}\right)\right]\Delta\phi\ .
    \end{split}
\end{equation}
In order to match \eqref{singsource} with \eqref{geneqm}, we first have impose $\vartheta=0$. Furthermore, we must take $d=-f$ and select the following parameters:
\be 
\begin{split}
    b=-2\left(1+2\gamma\right)\ ,\quad d=-f=2\left(1-\alpha-\frac{\gamma}{2}\right)\ ,\quad e=2\left(1-\alpha+\gamma\right)\ .
\end{split}
\ee
The above equations directly imply:
\be 
\gamma=-\frac{b+2}{4}\ ,\quad \alpha=\frac{10-4d+b}{8}\ .
\ee
Hence, $e$ too gets fixed in terms of $b$ and $d$ as:
\be 
e=\frac{2+4d+b}{4}\ .
\ee 
Therefore, the restricted flow 
\be\label{mf}
\begin{split}
         \frac{\de g_{\mu\nu}}{\de\lambda}&\equiv -2R_{\mu\nu}+ b\nabla_\mu\nabla_\nu\phi+g_{\mu\nu}d\Delta\phi\\
         &\quad+\frac{2+4d+b}{4}\nabla_\mu\phi\nabla_\nu\phi-dg_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi
\end{split}
\ee
can be derived as the volume-preserving metric gradient flow of the entropy $\mathcal{F}$-functional:
\begin{equation}
        \mathcal{F}\left(g,\phi\right)=\int\diff^{D}x\sqrt{g}e^{-\phi}\left[R+\frac{10-4d+b}{8}\left(\nabla\phi\right)^2-\frac{b+2}{4}\Delta\phi\right]\ .
\end{equation}
If we wanted to also consider the associated scalar flow, we would have:
\begin{equation}\label{sf}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-R+\left[\frac{4d-b-2}{8}\left(1-D\right)-\frac{b+2}{4}\left(1+\frac{D}{2}\right)\right]\left(\nabla\phi\right)^{2}+\\
        &-\left[1-D\frac{4d-b-2}{8}-\frac{b+2}{4}\left(2+\frac{D}{2}\right)\right]\Delta\phi\\
        &\equiv-R+f_D\left(\nabla\phi\right)^{2}-g_D\Delta\phi\ .
    \end{split}
\end{equation}
What would assuming \eqref{mf} and \eqref{sf} imply for the energy-momentum tensor $T_{\mu\nu}$? In order to investigate such question, we start from
\be 
T_{\mu\nu}=\nabla_\mu\phi\nabla_\nu\phi-g_{\mu\nu}\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi-\frac{m^2}{2}\phi^2\right)\ ,
\ee 
where $m$ is the mass of the scalar field $\phi$. By taking the $\lambda$-derivative, we have:
\be
\begin{split}\label{indflowT}
    \frac{\de T_{\mu\nu}}{\de\lambda}\equiv E_{\mu\nu}&=-\nabla_\mu\phi\nabla_\nu R+f_D\nabla_\mu\phi\nabla_\nu\left(\nabla\phi\right)^{2}-g_D\nabla_\mu\phi\nabla_\nu\Delta\phi\\
    &\quad-\nabla_\nu\phi\nabla_\mu R+f_D\nabla_\nu\phi\nabla_\mu\left(\nabla\phi\right)^{2}-g_D\nabla_\nu\phi\nabla_\mu\Delta\phi\\
    &\quad-g_{\mu\nu}m^2\phi\left[-R+f_D\left(\nabla\phi\right)^{2}-g_D\Delta\phi\right]\\
    &\quad+g_{\mu\nu}\left[\nabla^\alpha\phi\nabla_\alpha R-f_D\nabla^\alpha\phi\nabla_\alpha\left(\nabla\phi\right)^{2}+g_D\nabla^\alpha\phi\nabla_\alpha\Delta\phi\right]\\
    &\quad+2R_{\mu\nu}\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi-\frac{m^2}{2}\phi^2\right)\\
    &\quad- b\nabla_\mu\nabla_\nu\phi\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi-\frac{m^2}{2}\phi^2\right)\\
    &\quad-g_{\mu\nu}d\Delta\phi\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi-\frac{m^2}{2}\phi^2\right)\\
    &\quad-\frac{2+4d+b}{4}\nabla_\mu\phi\nabla_\nu\phi\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi-\frac{m^2}{2}\phi^2\right)\\
         &\quad+dg_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi-\frac{m^2}{2}\phi^2\right)\ .
\end{split}
\ee
By selecting a specific flow for the metric tensor, we have thus obtained it as the gradient flow from an $\mathcal{F}$-entropy functional. Therefore, we managed to derived the associated scalar flow equation. Such a discussion directly implies an energy-momentum tensor flow sourced by \eqref{indflowT}. Conversely, by selecting the same flow for the metric tensor and imposing Einstein field equations to be on-shell along the flow, we have obtained an explicit expression \eqref{osbssi} for the required flow source of the energy-momentum tensor. Being the two different, we will apply the procedure described in section \ref{entropysection} and try to account for it by introducing extra matter fields in specific examples.
%compute it, compare it with B_munu: different. Either we assume phi not to follow that gradient flow or we allow new fields to enter the theory. How do you estimate their contribution? Take the B_munu-dT_munu\dl difference as the evolution of this extra source, set it equal to zero at the beginning and see how it behaves. Maybe, study only its trace (properly)!
%take a specific solution, like the one in which the cosmological constant is sourced by a scalar. Apply the machinery and see what happens
\subsubsection{An example in $D=2$}\label{specific}
We now focus on a specific and simple example, which will allow us to derive explicit and insightful results. First of all, we assume to work in $D=2$, with coordinates $\left(t,x\right)$. This way we can take a very simple ansatz for our static metric:
\be 
g_{\mu\nu}=\begin{pmatrix}
-g_1\left(x\right) & 0 \\
a & g_2\left(x\right)
\end{pmatrix}
\ee
Moreover, we assume the scalar field to be time-independent. The fact that we work in $D=2$ implies that:
\be 
R_{\mu\nu}=\frac{R}{2}g_{\mu\nu}\ .
\ee
It can be easily shown that all the above assumptions are conserved along the flow. On top of that, the non-trivial Christoffel symbols are:
\be 
\Gamma^t_{\ tx}=\Gamma^t_{\ xt}=\frac{g_1'}{2g_1}\ ,\quad\Gamma^x_{\ tt}=\frac{g_1'}{2g_2}\ ,\quad\Gamma^x_{\ xx}=\frac{g_2'}{2g_2}\ .
\ee 
We simply have $\nabla_\alpha\phi\nabla^\alpha\phi=\left(\phi'\right)^2/g_2$, where the prime-symbol stands for an $x$-derivative. In order to make our setting even simpler, we choose $d=b=0$ in the flow source $A_{\mu\nu}$, so that also $f=0$ and $e=1/2$, consistently with the derivation of our flow equations from the $\mathcal{F}$-functional. So, they reduce to:
\be\label{specflmet}
\begin{split}
         \frac{\de g_{\mu\nu}}{\de\lambda}&= -2R_{\mu\nu}+\frac{1}{2}\nabla_\mu\phi\nabla_\nu\phi\ ,
\end{split}
\ee
\begin{equation}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-R-\frac{3}{4}\left(\nabla\phi\right)^{2}\ .
    \end{split}
\end{equation}
Before writing them explicitly in terms of $g_1$ and $g_2$, we observe that:
\be 
R=\frac{g_2 \left[\left(g_1'\right)^2-2 g_1 g_1''\right]+g_1 g_1'g_2'}{2 g_1^2 g_2^2}
\ee 
Therefore, the three equations are:
\be
\begin{split}
         \frac{\de g_1}{\de\lambda}= -\frac{g_2 \left[\left(g_1'\right)^2-2 g_1 g_1''\right]+g_1 g_1'g_2'}{2 g_1 g_2^2}=-Rg_1\ ,
\end{split}
\ee
\be
\begin{split}
         \frac{\de g_2}{\de\lambda}=\equiv -\frac{g_2 \left[\left(g_1'\right)^2-2 g_1 g_1''\right]+g_1 g_1'g_2'}{2 g_1^2 g_2}+\frac{\left(\phi'\right)^2}{2}=-Rg_2+\frac{\left(\phi'\right)^2}{2}\ ,
\end{split}
\ee
\begin{equation}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-\frac{g_2 \left[\left(g_1'\right)^2-2 g_1 g_1''\right]+g_1 g_1'g_2'}{2 g_1^2 g_2^2}-\frac{3\left(\phi'\right)^2}{4g_2}=-R-\frac{3\left(\phi'\right)^2}{4g_2}\ .
    \end{split}
\end{equation}
Concerning the differential operators appearing in $B_{\mu\nu}$, we have $\Omega_{\mu\nu}=0$,
\be
\Theta_{\mu\nu}=\frac{1}{2}\left(g_{\mu\nu}\Delta-\nabla_\mu\nabla_\nu \right)\ ,
\ee
and, finally:
\be
\begin{split}
   \Sigma_{\mu\nu}^{\sigma\theta }&=\frac{1}{2}\Big[\left(R_\mu{}^\sigma+\nabla_\mu\nabla^\sigma \right)\delta_\nu^{\ \theta}+g_{\mu\nu}R^{\sigma\theta}-g_{\mu\nu}\nabla^\sigma\nabla^\theta -R_\mu{}^\sigma{}_\nu {}^\theta\\
&\quad+\left(2\Lambda-R-\Delta \right)\delta_{\mu}^{\ \sigma}\delta_{\nu}^{\ \theta}+\delta_{\mu}^{\ \sigma}\nabla^\theta\nabla_\nu\Big] \ .
\end{split}
\ee
Since we are in $D=2$, we simply set $\Lambda=C=0$. Thus, the expression \eqref{osbssi} for $B_{\mu\nu}$ therefore becomes:
\be
\begin{split}
   2B_{\mu\nu}=\Theta_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi+\Sigma_{\mu\nu}^{\sigma\theta}\nabla_\sigma\phi\nabla_\theta\phi\ .
\end{split}
\ee
Making the last terms explicit, we have:
\be
\begin{split}
    2B_{\mu\nu}&=\frac{1}{2}\Big[\delta_\nu^{\ \theta}\nabla_\mu\nabla^\sigma -g_{\mu\nu}\nabla^\sigma\nabla^\theta +\delta_{\mu}^{\ \sigma}\nabla^\theta\nabla_\nu\Big]\nabla_\sigma\phi\nabla_\theta\phi\\
&\quad-\frac{R}{4}\nabla_\mu\phi\nabla_\nu\phi+\frac{1}{2}\left(g_{\mu\nu}\Delta-\nabla_\mu\nabla_\nu \right)\nabla_\alpha\phi\nabla^\alpha\phi\\
&\quad-\Delta\left(\nabla_\mu\phi\nabla_\nu\phi\right)\ .
\end{split}
\ee
For the sake of simplicity, we can further assume the scalar field to be massless. Concerning $E_{\mu\nu}$, we are hence left with:
\be
\begin{split}
E_{\mu\nu}&=-\nabla_\mu\phi\nabla_\nu R-\nabla_\nu\phi\nabla_\mu R-\frac{3}{4}\nabla_\mu\phi\nabla_\nu\left(\nabla\phi\right)^{2}\\
    &\quad-\frac{3}{4}\nabla_\nu\phi\nabla_\mu\left(\nabla\phi\right)^{2}+\left(R_{\mu\nu}-\frac{1}{4}\nabla_\mu\phi\nabla_\nu\phi\right)\nabla_\alpha\phi\nabla^\alpha\phi\\
    &\quad+g_{\mu\nu}\left[\nabla^\alpha\phi\nabla_\alpha R+\frac{3}{4}\nabla^\alpha\phi\nabla_\alpha\left(\nabla\phi\right)^{2}\right]\ .
\end{split}
\ee
From such expressions, we can obtain $S_{\mu\nu}$ as $E_{\mu\nu}-B_{\mu\nu}$:
\be
\begin{split}\label{2ds}
    S_{\mu\nu}&=-\nabla_\mu\phi\nabla_\nu R-\nabla_\nu\phi\nabla_\mu R-\frac{3}{2}\nabla_\mu\phi\nabla^\alpha\phi\nabla_\nu\nabla_\alpha\phi\\
    &\quad-\frac{3}{2}\nabla_\nu\phi\nabla^\alpha\phi\nabla_\mu\nabla_\alpha\phi-\frac{1}{4}\nabla_\mu\phi\nabla_\nu\phi\nabla_\alpha\phi\nabla^\alpha\phi\\
    &\quad+g_{\mu\nu}\left[\nabla^\alpha\phi\nabla_\alpha R+\frac{3}{2}\nabla^\alpha\phi\nabla^\beta\phi\nabla_\alpha\nabla_\beta\phi\right]\\
&\quad+\frac{R}{4}\nabla_\mu\phi\nabla_\nu\phi-g_{\mu\nu}\left(\nabla^\beta\nabla_\beta\nabla_\alpha\phi\nabla^\alpha\phi+\nabla^\beta\nabla_\alpha\phi\nabla_\beta\nabla^\alpha\phi\right)\\
&\quad+\nabla^\alpha\nabla_\alpha\nabla_\mu\phi\nabla_\nu\phi+2\nabla^\alpha\nabla_\mu\phi\nabla_\alpha\nabla_\nu\phi\\
&\quad +\nabla_\mu\nabla_\nu\nabla_\alpha\phi\nabla^\alpha\phi+\nabla_\nu\nabla_\alpha\phi\nabla_\mu\nabla^\alpha\phi+\nabla_\mu\phi\nabla^\alpha\nabla_\alpha\nabla_\nu\phi\\
&\quad-\frac{1}{2}\nabla_\mu\phi\nabla^\theta\nabla_\nu\nabla_\theta\phi-\frac{1}{2}\nabla_\sigma\phi\nabla_\mu\nabla^\sigma\nabla_\nu\phi\\
&\quad -\frac{1}{2}\nabla^\theta\nabla_\nu\nabla_\mu\phi\nabla_\theta\phi-\frac{1}{2}\nabla_\nu\nabla_\mu\phi\nabla^\theta\nabla_\theta\phi-\frac{1}{2}\nabla^\theta\nabla_\mu\phi\nabla_\nu\nabla_\theta\phi\\
&\quad-\frac{1}{2}\nabla_\mu\nabla^\sigma\nabla_\sigma\phi\nabla_\nu\phi-\frac{1}{2}\nabla^\sigma\nabla_\sigma\phi\nabla_\mu\nabla_\nu\phi-\frac{1}{2}\nabla_\mu\nabla_\sigma\phi\nabla^\sigma\nabla_\nu\phi\\
&\quad+\frac{1}{2}g_{\mu\nu} \Big(\nabla^\sigma\nabla^\theta\nabla_\sigma\phi\nabla_\theta\phi+\nabla^\theta\nabla_\sigma\phi\nabla^\sigma\nabla_\theta\phi+\nabla^\sigma\nabla_\sigma\phi\nabla^\theta\nabla_\theta\phi\\
&\quad+\nabla_\sigma\phi\nabla^\sigma\nabla^\theta\nabla_\theta\phi\Big)\ .
\end{split}
\ee
Clearly, the expression \eqref{2ds} is still too complicated to be treated nicely. In order to simplify it, we refer to the explicit computations performed in \ref{app2d}. Such derivations allow us to observe that $\nabla_\alpha\nabla_\beta\phi=\nabla_\beta\nabla_\alpha\phi$. By exploiting such symmetry, we get:
\be
\begin{split}\label{2dssimp}
    S_{\mu\nu}&=-\nabla_\mu\phi\nabla_\nu R-\nabla_\nu\phi\nabla_\mu R-\frac{3}{2}\nabla_\mu\phi\nabla^\alpha\phi\nabla_\nu\nabla_\alpha\phi\\
    &\quad-\frac{3}{2}\nabla_\nu\phi\nabla^\alpha\phi\nabla_\mu\nabla_\alpha\phi-\frac{1}{4}\nabla_\mu\phi\nabla_\nu\phi\nabla_\alpha\phi\nabla^\alpha\phi\\
    &\quad+g_{\mu\nu}\left(\nabla^\alpha\phi\nabla_\alpha R+\frac{3}{2}\nabla^\alpha\phi\nabla^\beta\phi\nabla_\alpha\nabla_\beta\phi\right)\\
&\quad+\frac{R}{4}\nabla_\mu\phi\nabla_\nu\phi+\Delta\nabla_\mu\phi\nabla_\nu\phi+2\nabla^\alpha\nabla_\mu\phi\nabla_\alpha\nabla_\nu\phi\\
&\quad +\frac{1}{2}\nabla_\mu\nabla_\nu\nabla_\alpha\phi\nabla^\alpha\phi+\frac{1}{2}\nabla_\mu\phi\Delta\nabla_\nu\phi\\
&\quad -\frac{1}{2}\nabla^\theta\nabla_\nu\nabla_\mu\phi\nabla_\theta\phi-\nabla_\nu\nabla_\mu\phi\Delta\phi-\frac{1}{2}\nabla_\mu\Delta\phi\nabla_\nu\phi\\
&\quad+\frac{1}{2}g_{\mu\nu} \Big(\Delta\phi\Delta\phi+\nabla_\sigma\phi\nabla^\sigma\Delta\phi-\Delta\nabla^\theta\phi\nabla_\theta\phi-\nabla^\theta\nabla_\sigma\phi\nabla^\sigma\nabla_\theta\phi\Big)\ .
\end{split}
\ee
By assuming both $R$ and the initial scalar configuration to be constant, we have that such conditions are conserved along the whole flow. So, we get that $S_{\mu\nu}$ simplifies to:
\be
\begin{split}
    S_{\mu\nu}&=0\ .
\end{split}
\ee
At this point, we an explicitly solve the flow equations. We do so by taking the metric to be that of $2$-dimensional (Anti-)de Sitter spacetime
\be 
g_{1}=1-\frac{\kappa x^2}{2}\ ,\quad g_{2}=\frac{1}{g_1}
\ee 
for which we simply have:
\be 
R=\kappa\ .
\ee
From the flow equation \eqref{specflmet} and the assumption of having a spacetime-constant scalar field, we can derive the flow equation
\be 
\frac{\de R}{\de\lambda}=R^2
\ee
for the Ricci scalar $R$, which can be solved explicitly as:
\be 
R\left(\lambda\right)=\frac{R_0}{1-R_0\lambda}\ .
\ee
As is well-known from previous works \cite{Kehagias:2019akr,DeBiasio:2020xkv}, it is well known that:
\begin{itemize}
    \item When $R_0>0$, the evolution reaches a singularity at a finite flow time.
    \item When $R_0<0$, the evolution asymptotically flows to flat spacetime.
\end{itemize}
Thus, we have:
\be 
\kappa\left(\lambda\right)=\frac{\kappa_0}{1-\kappa_0\lambda}\ .
\ee 
Concerning the scalar flow equation
\be 
\frac{\de\phi}{\de\lambda}=-R\ ,
\ee 
we can solve it and get:
\be 
\phi\left(\lambda\right)=\phi_0+\int_0^\lambda\frac{\kappa_0}{\kappa_0\tau-1}\diff\tau=\phi_0+\log{\left(1-\kappa_0\lambda\right)}\ .
\ee 
Since $S_{\mu\nu}=0$, the $2$-dimensional example gives us no interesting behaviour. This is something that should have been expected. Indeed, general relativity is trivial in $D=2$ and the energy-momentum tensor for a constant scalar is null.

\subsubsection{An example in $D=3$}\label{specific2}
In the following discussion, we reproduce the analysis performed in \ref{specific} in the case in which $D=3$. In order to do so, we once more assume to work with an initial condition comprised of the metric of an Einstein manifold -more specifically, that of Anti de-Sitter spacetime in $D=3$- and a massless, scalar field with constant spacetime value $\phi_0$. 
By assuming, once more, $d=b=0$ in the flow equations, we are left with:
\be
\begin{split}
 \frac{\de g_{\mu\nu}}{\de\lambda}= -2R_{\mu\nu}+\frac{1}{2}\nabla_\mu\phi\nabla_\nu\phi\ ,\quad   
  \frac{\de\phi}{\de\lambda}=-R-\frac{3}{4}\left(\nabla\phi\right)^{2}\ .
\end{split}
\ee
Such equations conserve our assumptions on $g_{\mu\nu}$ and $\phi$, so that we get
\be
\frac{\de R}{\de\lambda}=\frac{2R^2}{3}\ ,\quad \frac{\de\phi}{\de\lambda}=-R\ ,
\ee
precisely as in \ref{specific}, except for a small deviation due to different dimensionality. 
By already removing the terms containing derivatives of $\phi$, plugging-in the expression of $R_{\mu\nu}$ in terms of $R$ and $g_{\mu\nu}$ and remembering Anti-de Sitter spacetime scalar curvature is linked to the cosmological constant $\Lambda$ by
\be \label{equal}
R=6\Lambda
\ee
the expression for $S_{\mu\nu}$ gets to be:
\be
\begin{split}
   S_{\mu\nu}&=\left(4\Lambda^2-C\right)g_{\mu\nu}\ .
\end{split}
\ee
Therefore, the flow equation for the emergent energy-momentum tensor $\hat{T}_{\mu\nu}$ is:
\be
\frac{\de\hat{T}_{\mu\nu}}{\de\lambda}=\left(4\Lambda^2-C\right)g_{\mu\nu}\.
\ee
Plugging-in an ansatz of the form
\be
\hat{T}_{\mu\nu}=\frac{\hat{T}}{3}g_{\mu\nu}\ ,
\ee
our equation simply reduces to:
\be
\frac{\de\hat{T}}{\de\lambda}=3\left(4\Lambda^2-C\right)\ .
\ee
By imposing the initial condition $\hat{T}_{\mu\nu}=0$ and remembering that $C$ appeared as the flow-source for $\Lambda$, we can solve the above equation as:
\be
\hat{T}\left(\lambda\right)=12\int_0^\lambda\Lambda^2\left(\tau\right)\diff\tau-3\left[\Lambda\left(\lambda\right)-\Lambda_0\right]\ .
\ee
In the following, we will explore three natural behaviours for $\Lambda$. First of all, we can take it to be constant in the flow parameter. Hence, we have:
\be
\hat{T}\left(\lambda\right)=12\Lambda^2\lambda\ .
\ee
If we instead take $\Lambda$ to be exponentially dropping as
\be 
\Lambda\left(\lambda\right)=\Lambda_0e^{-\lambda}\ ,
\ee
we would get:
\be
\hat{T}\left(\lambda\right)=6\Lambda_0^2\left(1-e^{-2\lambda}\right)+3\Lambda_0\left(1-e^{-\lambda}\right)\ .
\ee
For large values of the flow parameter, we get:
\be 
\hat{T}\left(\lambda\right)=3\Lambda_0\left(2\Lambda_0+1\right)\ .
\ee 
By assuming $\Lambda_0=-1$, this would imply the behaviour depicted in figure \ref{fig}. 
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{That.png}
    \caption{Plot of $\hat{T}$ against the flow parameter $\lambda$.}
    \label{fig}
\end{figure}
Last, we must consider the case in which the \eqref{equal} is taken to hold for the whole flow. Thus, $S_{\mu\nu}=0$ and no extra energy-momentum tensor $\hat{T}_{\mu\nu}$ emerges. Generally speaking and assuming any emergent field to be a real scalar, an energy-momentum tensor satisfying $\hat{T}_{\mu\nu}=\frac{\hat{T}}{3}g_{\mu\nu}$ can only be achieved by imposing
\be
\hat{T}=-\sum_{k=1}^{M}\frac{3m_k^2}{2}\phi_k^2\ ,
\ee
where $\phi_k$ are $M$ emergent spacetime-constant fields, which we will from now on normalise to $\phi_k=\sqrt{2/3}$, and $m_k$ the corresponding mass scales. Thus, we get:
\be
\hat{T}=-\sum_{k=1}^{M}m_k^2\ .
\ee
Therefore, making such masses flow-dependent, we have:
\be 
\sum_{k=1}^{M}m_k^2\left(\lambda\right)=3\left[\Lambda\left(\lambda\right)-\Lambda_0\right]-12\int_0^\lambda\Lambda^2\left(\tau\right)\diff\tau\ .
\ee
Taking the masses to be distributed as 
\be
m_k=m\sqrt{n}
\ee
and assuming only a finite portion of them to enter the theory, we would get:
\be 
m^2\left(\lambda\right)=\frac{3}{C_M}\left[\Lambda\left(\lambda\right)-\Lambda_0\right]-\frac{12}{C_M}\int_0^\lambda\Lambda^2\left(\tau\right)\diff\tau\ ,
\ee
where the numerical constant is
\be
C_M\equiv \frac{M(M+1)}{2}
\ee
and depends on the number of extra fields we choose to include in the theory.
%\be
%\frac{1}{\alpha^2}=\frac{2\Lambda}{(1-D)(D-2)}
%\ee

\subsection{Single self-interacting scalar field}\label{potentialcase}

In the following discussion, we assume to work with a single scalar field $\phi$, subject to a potential of the form
\be \label{6pot}
V\left(\phi\right)=\frac{V_0}{\alpha_0}\phi^2\left(\phi^4-9\phi^2+21\right)\ ,
\ee
with $\alpha_0=9-4\sqrt{2}$, so that the values of the potential minima of our interest are normalised to $V_0$, which is taken to be a positive parameter. The potential is shown in figure \ref{pottV}.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{V.png}
    \caption{Plot of the behaviour of $V\left(\phi\right)$ around $\phi=0$, when $V_0=1$.}
    \label{pottV}
\end{figure}
This can be achieved as a simple and straightforward generalisation of the discussion developed at the beginning of section \ref{scaler}, in which the only thing to be altered is the specific form of the energy-momentum tensor:
\be
T_{\mu\nu}=\nabla_\mu\phi\nabla_\nu\phi-g_{\mu\nu}\left[\frac{1}{2}\nabla^\alpha\phi\nabla_\alpha\phi-V\left(\phi\right)\right]\ .
\ee
The equations of motion for $\phi$ can be solved by taking the scalar to have the spacetime-constant value $\phi_0$, corresponding to a minimum of the potential. This will serve as our initial flow configuration, together with an appropriate solution for the metric. Since the potential will produce an effective cosmological constant term
\be
\Lambda_{\text{eff}}=-V_0\ ,
\ee
we take $\Lambda=C=0$ and simplify the whole discussion. Therefore, our initial metric will be that of $D$-dimensional Anti-de Sitter spacetime with scalar curvature:
\be 
R=\frac{2D}{D-2}\Lambda_{\text{eff}}=\frac{2D}{2-D}V_0\ .
\ee
Since we have taken the scalar to be spacetime constant at the starting point of the flow, both this condition and the metric being that of Anti-de Sitter spacetime are conserved along the flow. Hence, by taking $d=b=0$, the flow equations reduce to:
\be 
\frac{\de R}{\de\lambda}=\frac{2R^2}{D}\ ,\quad \frac{\de\phi}{\de\lambda}=-R\ .
\ee 
By solving the equations, as we did in the previous examples, we get
\be 
R\left(\lambda\right)=\frac{DR_0}{D-R_02\lambda}\ ,\quad \phi\left(\lambda\right)=\phi_0+\frac{D}{2}\log\left(1-\frac{2R_0\lambda}{D}\right)\ ,
\ee
where we have defined
\be 
\phi_0\equiv\sqrt{3+\sqrt{2}}\ ,
\ee
so that it corresponds to the potential minimum $V\left(\phi_0\right)=V_0$. For the rest of the discussion, we take $V_0=1$ and have our flow behaviours reduce to:
\be 
R\left(\lambda\right)=\frac{2D^2}{D(2-D)-4D\lambda}\ ,\quad \phi\left(\lambda\right)=\phi_0+\frac{D}{2}\log\left(1+\frac{4\lambda}{D-2}\right)\ ,
\ee
Figure \ref{flowbeh} shows them explicitly against $\lambda$.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{GG.png}
    \caption{Plot of the flow behaviour of $R$ and $\phi$, in $D=4$. For large values of the flow parameter, we have $R\to 0$ and $\phi\to\infty$.}
    \label{flowbeh}
\end{figure}
It can be straightforwardly shown that:
\be
\begin{split}
   E_{\mu\nu}&=g_{\mu\nu}\frac{\de V\left(\varphi\right)}{\de\varphi}\Bigg|_{\varphi=\phi}\cdot\frac{\de\phi}{\de\lambda}+\frac{\de g_{\mu\nu}}{\de\lambda}V\left(\phi\right) \\
   &=-\frac{2R\phi}{D\alpha_0}g_{\mu\nu}\left(\phi^5+3D\phi^4-9\phi^3-18D\phi^2+21\phi+21D\right)\ .
\end{split}
\ee
\be 
\begin{split}
    B_{\mu\nu}&=0\ .
\end{split}
\ee
Concerning the flow of the extra energy-momentum tensor term, we hence obtain
\be
S_{\mu\nu}=C_0g_{\mu\nu}\ ,
\ee
where we have defined:
\be
\begin{split}
    C_0&=\frac{2R\phi}{D\alpha_0}\left(\phi^5+3D\phi^4-9\phi^3-18D\phi^2+21\phi+21D\right)\ .
\end{split}
\ee
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{C.png}
    \caption{Plot of the flow behaviour of $C_0$ for different values of the dimension $D$.}
    \label{czer}
\end{figure}
At this point, we can take the extra energy momentum tensor to be of the form
\be
\hat{T}_{\mu\nu}=\Omega g_{\mu\nu}\ ,
\ee
in which $\Omega$ follows the flow equation:
\be 
\frac{\de\Omega}{\de\lambda}=C_0\ .
\ee
Being $C_{0}$, as in figure \ref{czer}, negative for every value of $\lambda$, we have that $\Omega$, with the initial condition $\Omega_0=0$, is negative too, with its absolute value growing along the flow as shown in figure \ref{omegaa}. If we want this feature to be accounted for by the appearance of some extra fields, the most natural way to achieve this behaviour for $\Omega$ is the following. Let's assume the states to be labelled as $\varphi_k$ and to sit at the minimum of some potential $\hat{V}$, in which we include mass terms for the states, so that it takes the value
\be 
\hat{V}\left(\lambda\right)=\hat{V}_{\text{min}}+\sum_{k=1}^K\frac{m^2_k\left(\lambda\right)}{2}\ ,
\ee
where the whole flow dependence was moved to the masses. Now, let's assume all the $\varphi_k$ to be spacetime constant. They contribute to $\hat{T}_{\mu\nu}$ as:
\be 
\hat{T}_{\mu\nu}\left(\lambda\right)=\hat{V}\left(\lambda\right)g_{\mu\nu}\ .
\ee
Therefore, we must have:
\be 
\hat{V}\left(\lambda\right)=\Omega\left(\lambda\right)\ .
\ee
Since the fields do not appear in the theory at $\lambda=0$, their masses should be high. This straightforwardly implies $\hat{V}_{\text{min}}$ to be negative, so that $\hat{V}\left(0\right)=0$ as expected from the equivalence with $\Omega\left(\lambda\right)$, that must hold for any value of the flow parameter. Thus, for $\Omega\left(\lambda\right)$ to have the flow behaviour derived in our discussion, we must take the masses contribution to $\hat{V}\left(\lambda\right)$ to decrease with $\lambda$. Namely, we have a tower of masses getting lighter with the flow. Concerning the specific value of $\hat{V}_{\text{min}}$, we can expect to read it off from the asymptotic behaviour of $\Omega\left(\lambda\right)$, as the masses contribution drops to zero. There, we know that $C_0$ tends to zero since the drop of the $R$ factor dominates the growth of the $\phi$-polinomial. Hence, we can reasonably expect $\Omega\left(\lambda\right)$ to tend to a negative constant, precisely equal to $\hat{V}_{\text{min}}$. Therefore, as our Anti-de Sitter spacetime flows to flat Minkowski and as our scalar blows to infinity with a logarithmic behaviour, according to the appropriate gradient flow equations that -in this case- match with Perelman's combined flow, the requirement of the equations of motion for the metric to be on-shell forces a tower of states to appear in the low energy theory. This is not only consistent with the naive prediction of a reasoning qualitatively tied to the Swampland distance conjecture, but also holds in general dimension. No statement can be made on the flow behaviour of the specific mass of one of such states, since they collectively realise $\Omega$. Addressing such question could make for a natural prosecution of the current work and would allow us to better connect it to the distance conjecture.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Omega.png}
    \caption{Plot of the flow behaviour of $\Omega$ when $D=4$ is assumed.}
    \label{omegaa}
\end{figure}
%Here I might add a small discussion in which I consider the flow equations induced by the action, rather than the ones coming from an arbitrary entropy functional, as discussed in "Geometric flow of bubbles". The idea would be the following: take the example, derive the flow equations using the explicit form of the potential, apply them to our solution and see what this implies for the energy-momentum tensor from on-shell requirements. Then, derive the flow equation for T from that of phi and conclude the discussion by showing how S produces whatever it produces for \hat{T}
\subsubsection{Flow equations from the action}
In the following discussion, we will once more consider the initial metric and scalar configuration introduced in \ref{potentialcase}. Namely, we work with a $D$-dimensional Anti-de Sitter spacetime geometry, whose curvature is sourced by the spacetime constant value of a scalar $\phi$, sitting at the appropriate minimum of the potential \eqref{6pot}. Indeed, we have
\be 
\phi_0\equiv\sqrt{3+\sqrt{2}}\ ,\quad R_0=-\frac{2D}{D-2}\ ,
\ee
where we have once more taken $V_0=1$. Moreover, we assume $D>2$. The main change with respect to the previous analysis is that we consider a different set of flow equations. In particular, exploiting the general results described in \cite{DeBiasio:2022omq}, we derive a system of gradient flow equations from a new entropy-$\mathcal{F}$ functional, obtained as the euclidean string-frame version of the action of our theory. This way, the introduction of the potential \eqref{6pot} directly influences the expression for the flow equations. In the above-mentioned reference, it was shown that an action
\begin{equation}\label{aact}
    S=\int\diff^{D}x\sqrt{\tilde{g}}\left[\tilde{R}+\frac{1}{2}\left(\nabla \phi\right)^{2}-\sum_{n=0}^{+\infty}\frac{g_{n}}{n!}\phi^{n}\right]\ .
\end{equation}
naturally induces, neglecting the diffeomorphism term, the flow equations
\begin{equation}\label{acteq}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}-g_{\mu\nu}\sum_{n=1}^{+\infty}ns_{\ n}^{(D)}\phi^{n-1}+4\frac{D-1}{D-2}\nabla_{\mu}\phi\nabla_{\nu}\phi\\
        &-2\frac{5D-6}{D-2}\nabla_{\nu}\nabla_{\mu}\phi-2\frac{D-1}{D-2}g_{\mu\nu}\nabla^{2}\phi+2\frac{D-1}{D-2}g_{\mu\nu}\left(\nabla \phi\right)^2\ ,\\
        \frac{\de \phi}{\de\lambda}=&-R-\frac{D}{2}\sum_{n=1}^{+\infty}ns_{\ n}^{(D)} \phi^{n-1}+\frac{\left(D-1\right)\left(D+2\right)}{D-2}\left(\nabla \phi\right)^{2}\\
        &-\frac{D^{2}+4D-6}{D-2}\nabla^{2} \phi\ ,
    \end{split}
\end{equation}
where the $s_{\ k}^{(D)}$ parameters have been defined as:
\be 
    s_{\ k}^{(D)}\equiv\sum_{n=0}^{k}\frac{g_{n}}{\left(k-n\right)!n!}\left(\frac{2}{2-D}\right)^{k-n}\left(\frac{4D-6}{D-2}\right)^{n/2}\ .
\ee
For the specific case of the potential
\be
V\left(\phi\right)=\frac{1}{\alpha_0}\phi^2\left(\phi^4-9\phi^2+21\right)\ ,
\ee
with $\alpha_0=9-4\sqrt{2}$, we have:
\be
g_2=\frac{42}{\alpha_0}\ ,\quad g_4=-\frac{9\cdot4!}{\alpha_0}\ ,\quad g_6=\frac{6!}{\alpha_0}\ .
\ee
Hence, the $s_{\ k}^{(D)}$ parameters are:
\be
\begin{split}
    s_{\ 0}^{(D)}&=s_{\ 1}^{(D)}=0\ ,\quad s_{\ 2}^{(D)}=\frac{42}{\alpha_0}\cdot\frac{2D-3}{D-2}\ ,\quad
    s_{\ 3}^{(D)}=-\frac{84}{\alpha_0}\cdot\frac{2D-3}{\left(D-2\right)^2}\ ,\\ s_{\ 4}^{(D)}&=-\frac{12}{\alpha_0}\cdot\frac{2D-3}{\left(D-2\right)^3}\left(6D^2-21D+11\right)\ ,\\
    s_{\ 5}^{(D)}&=\frac{8}{\alpha_0}\cdot\frac{2D-3}{(D-2)^4}\left(18D^2-27D-36D+47\right)\ ,\\
    s_{\ k\geq 6}^{(D)}&=\frac{(-1)^k2^{k-3}}{\left(k-6\right)!\alpha_0}\cdot\frac{2D-3}{(D-2)^{k-3}}\Bigg[
    \frac{84\left(k-6\right)!}{\left(k-2\right)!(D-2)^2}\\
    &\quad-\frac{9\left(k-6\right)!\left(4D-6\right)}{\left(k-4\right)!(D-2)}+\left(2D-3\right)^{2}\Bigg]\ .
\end{split}
\ee
Defining the simpler parameters
\be 
g_{\ k}^{(D)}\equiv\alpha_0s_{\ k}^{(D)}
\ee
and taking $D=4$ for the sake of simplicity, we get:
\be
\begin{split}
    g_{\ 0}^{(4)}&=g_{\ 1}^{(4)}=0\ ,\quad g_{\ 2}^{(4)}=105\ ,\quad
    g_{\ 3}^{(4)}=-105\ ,\\ g_{\ 4}^{(4)}&=-\frac{345}{2}\ ,\quad g_{\ 5}^{(4)}=\frac{415}{2}\ ,\\
g_{\ k\geq6}^{(4)}&=(-1)^k\Bigg[
    \frac{105}{\left(k-2\right)!}-\frac{225}{\left(k-4\right)!}+\frac{125}{\left(k-6\right)!}\Bigg]\ .
\end{split}
\ee
The explicit $k$-behaviour of such factors is shown in figure \ref{ddott}.
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{dotspl.png}
    \caption{Plot of $g_{\ k}^{(4)}$ for different values of $k$, at $D=4$. Clearly, the coefficients drop to zero in an extremely quick way.}
    \label{ddott}
\end{figure}
At this point, we must compute the value of the function:
\be 
F\left(\phi\right)\equiv \sum_{n=1}^{+\infty}ns_{\ n}^{(4)} \phi^{n-1}\ .
\ee
Therefore, we have:
\be 
\begin{split}
    \alpha_0F\left(\phi\right)&=210\phi-315\phi^2-690\phi^3+\frac{2075}{2}\phi^4\\
    &\quad+\sum_{k=6}^{+\infty}k(-1)^k\Bigg[
    \frac{105}{\left(k-2\right)!}-\frac{225}{\left(k-4\right)!}+\frac{125}{\left(k-6\right)!}\Bigg]\phi^{k-1}\\
    &=210\phi-315\phi^2-690\phi^3+\frac{2075}{2}\phi^4\\
    &\quad+105\phi\left[2\sum_{n=4}^{+\infty}\frac{(-\phi)^n}{n!}-\phi\sum_{l=3}^{+\infty}
    \frac{(-\phi)^l}{l!}\right]\\
    &\quad-225\phi^3\left[4\sum_{n=2}^{+\infty}\frac{(-\phi)^n}{n!}-\phi\sum_{l=1}^{+\infty}\frac{(-\phi)^{l}}{l!}\right]\\
    &\quad+125\phi^5\left[6\sum_{n=0}^{+\infty}\frac{(-\phi)^n}{n!}-\phi\sum_{l=0}^{+\infty}\frac{(-\phi)^l}{l!}\right]\\
    &=210\phi-315\phi^2-690\phi^3+\frac{2075}{2}\phi^4\\
    &\quad+105\phi\left[\left(2-\phi\right)\left(e^{-\phi}-1+\phi-\frac{\phi^2}{2}\right)+\frac{\phi^3}{3}\right]\\
    &\quad-225\phi^3\left[\left(4-\phi\right)\left(e^{-\phi}-1\right)+4\phi\right]+125\phi^5\left(6-\phi \right)e^{-\phi}\\
   &=5\left[42\phi-21\phi^2-220\phi^3+55\phi^4+150\phi^5-25\phi^6\right]e^{-\phi}\ .
\end{split}
\ee
In the end, we get:
\be
F\left(\phi\right)=\frac{5}{\alpha_0}\left[42\phi-21\phi^2-220\phi^3+55\phi^4+150\phi^5-25\phi^6\right]e^{-\phi}\ .
\ee
The plot of such a function is given in figure \ref{Fpl}. Given that
we start with constant curvature and scalar field, it can be shown that the flow equations \eqref{acteq} preserve such conditions. Thus, they reduce to:
\begin{equation}
    \begin{split}
        \frac{\de R}{\de\lambda}=&-\frac{R}{2}\left[R+2F\left(\phi\right)\right]\ ,\\
        \frac{\de \phi}{\de\lambda}=&-\left[R+2F\left(\phi\right)\right]\ .
    \end{split}
\end{equation}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{FFF.png}
    \caption{Plot of F against $\phi$, in which the exponential suppression can be observed.}
    \label{Fpl}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Flow.png}
    \caption{Flow behaviour for $R$ and $\phi$.}
    \label{fflo}
\end{figure}
Given the $D=4$ initial conditions
\be 
\phi_0\equiv\sqrt{3+\sqrt{2}}\ ,\quad R_0=-4\ ,
\ee
the flow can be straightforwardly solved numerically, as shown in figure \ref{fflo}. More generally, figure \ref{vec} shows the vector fields tangent to the flow, in the $\left(R,\phi\right)$ space.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Vector.png}
    \caption{Plot of the vector field tangent to the flow, in the $\left(R,\phi\right)$ space.}
    \label{vec}
\end{figure}
As in the previous derivation, we have $B_{\mu\nu}$ and
\be 
S_{\mu\nu}=C_0g_{\mu\nu}\ ,
\ee
with:
\be
\begin{split}
   C_0&=-\frac{1}{\alpha_0 }\left(\phi^6+12\phi^5-9\phi^4-72\phi^3+21\phi^2+84\phi\right)\left[\frac{R}{2}+F\left(\phi\right)\right]\ .
\end{split}
\ee
In figure \ref{ssoss}, the explicit flow behaviour of $C_0$ is shown. There we can observe that, after having grown to big positive values, it goes to negative ones and then tends to zero. 
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{GGGG.png}
    \caption{Plot of $C_0$ against the flow parameter $\lambda$.}
    \label{ssoss}
\end{figure}
By defining 
\be 
\hat{T}_{\mu\nu}=\Omega g_{\mu\nu}\ ,
\ee
we can expect $\Omega$ to reach a constant, positive value. Exploring the implication of such a result would require us to better understand the physical meaning of our action-induced flow equations. This goes beyond the scope of the current work.



==> swampcomm.tex <==
If we want this feature to be accounted for by the appearance of some extra fields, the most natural way to achieve this behaviour for $\Omega$ is the following. Let's assume the states to be labelled as $\varphi_k$ and to sit at the minimum of some potential $\hat{V}$, in which we include mass terms for the states, so that it takes the value
\be 
\hat{V}\left(\lambda\right)=\hat{V}_{\text{min}}+\sum_{k=1}^K\frac{m^2_k\left(\lambda\right)}{2}\ ,
\ee
where the whole flow dependence was moved to the masses. Now, let's assume all the $\varphi_k$ to be spacetime constant. They contribute to $\hat{T}_{\mu\nu}$ as:
\be 
\hat{T}_{\mu\nu}\left(\lambda\right)=\hat{V}\left(\lambda\right)g_{\mu\nu}\ .
\ee
Therefore, we must have:
\be 
\hat{V}\left(\lambda\right)=\Omega\left(\lambda\right)\ .
\ee
Since the fields do not appear in the theory at $\lambda=0$, their masses should be high. This straightforwardly implies $\hat{V}_{\text{min}}$ to be negative, so that $\hat{V}\left(0\right)=0$ as expected from the equivalence with $\Omega\left(\lambda\right)$, that must hold for any value of the flow parameter. Thus, for $\Omega\left(\lambda\right)$ to have the flow behaviour derived in our discussion, we must take the masses contribution to $\hat{V}\left(\lambda\right)$ to decrease with $\lambda$. Namely, we have a tower of masses getting lighter with the flow. Concerning the specific value of $\hat{V}_{\text{min}}$, we can read it off from the asymptotic value $\Omega_\infty\sim -1.52$ of $\Omega\left(\lambda\right)$, as the masses contribution drops to zero. Therefore, as our de Sitter spacetime curvature and our scalar flow to their asymptotic values, according to the appropriate gradient flow equations derived from the theory action, the requirement of the equations of motion for the metric to be on-shell forces a tower of states to appear in the low energy theory. This is consistent with the naive prediction of a reasoning qualitatively tied to the Swampland distance conjecture. No statement can be made on the flow behaviour of the specific mass of one of such states, since they collectively realise $\Omega$. Addressing such question could make for a natural prosecution of the current work and would allow us to better connect it to the distance conjecture.







Albeit still being an extremely simplified setting, the last one allowed us to highlight the main features one would expect if the distance conjecture, together with the requirement of the metric to be on-shell, was taken to hold true. Namely, we found that massive states represent the most natural candidate for the extra energy-momentum tensor terms appearing due to action-induced geometric flow equations. 
